Supporting Capabilities For Underground Facilities

The 2021 particle physics community study, known as "Snowmass 2021", has brought together particle physicists around the world to create a unified vision for the field over the next decade. One of the areas of focus is the Underground Facilities (UF) frontier, which addresses underground infrastructure and the scientific programs and goals of underground-based experiments. To this effect, the UF Supporting Capabilities topical group created two surveys for the community to identify potential gaps between the supporting capabilities of facilities and those needed by current and future experiments. Capabilities surveyed are discussed in this report and include underground cleanroom space size and specifications, radon-reduced space needs and availability, the assay need and other underground space needs as well timeline for future experiments. Results indicate that future, larger experiments will increasingly require underground assembly in larger, cleaner cleanrooms, often with better radon-reduction systems and increased monitoring capability for ambient contaminants. Most assay needs may be met by existing worldwide capabilities with organized cooperation between facilities and experiments. Improved assay sensitivity is needed for assays of bulk and surface radioactivity for some materials for some experiments, and would be highly beneficial for radon emanation.

==> usebiblatex.tex <==
\usepackage[backend=biber,style=numeric,citestyle=numeric-comp,giveninits=true,isbn=false,date=year,sorting=none]{biblatex}
% suppress `In:' from articles
\renewbibmacro{in:}{%
  \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
% ignore the number in the issue
\AtEveryBibitem{%
  \clearfield{number}}
% only print URL or arxiv if no DOI
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map[overwrite]{
      \step[fieldsource=doi, final]
      \step[fieldset=url, null]
      \step[fieldset=eprint, null]
    }  
  }
}
\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map[overwrite]{
      \step[fieldsource=eprint, final]
      \step[fieldset=url, null]
    }  
  }
}
\addbibresource{references.bib}

